Resilience: A Criterion for Learning in the Presence of Arbitrary Outliers

We introduce a criterion, resilience, which allows properties of a dataset (such as its mean or best low rank approximation) to be robustly computed, even in the presence of a large fraction of arbitrary additional data. Resilience is a weaker condition than most other properties considered so far in the literature, and yet enables robust estimation in a broader variety of settings. We provide new information-theoretic results on robust distribution learning, robust estimation of stochastic block models, and robust mean estimation under bounded $k$th moments. We also provide new algorithmic results on robust distribution learning, as well as robust mean estimation in $\ell_p$-norms. Among our proof techniques is a method for pruning a high-dimensional distribution with bounded $1$st moments to a stable "core" with bounded $2$nd moments, which may be of independent interest.

==> alg-recover-l2-2e.tex <==
\begin{algorithm}[t!]
\caption{Algorithm for recovering the mean of a set with bounded $2$nd moments in $\ell_2$-norm.}
\label{alg:recover-l2}
\SetAlgoLined
Initialize $c_i = 1$ for all $i=1,\ldots,n$ and $\sA = \{1,\ldots,n\}$.\;

Let $Y \in \bR^{d \times d}$ and $W \in \bR^{\sA \times \sA}$ 
be the maximizer/minimizer of the saddle point problem
\label{line:begin-loop}
  \begin{equation}
  \label{eq:opt-2}
  \max_{\substack{Y \succeq 0, \\ \tr(Y) \leq 1}} \min_{\substack{0 \leq W_{ij} \leq \frac{4-\alpha}{\alpha(2+\alpha) n}, \\ \sum_i W_{ij} \leq 1}} \sum_{i \in \sA} c_i (x_i - X_{\sA}w_i)^{\top}Y(x_i - X_{\sA}w_i).
  \end{equation}\;
\If{$\sum_{i \in \sA} c_i(x_i - X_{\sA}w_i)^{\top}Y(x_i - X_{\sA}w_i) > 4n\sigma^2$}{
\protect\label{line:if}
  Let $\tau_i = (x_i - X_{\sA}w_i)^{\top}Y(x_i - X_{\sA}w_i)$.\;

  For $i \in \sA$, replace $c_i$ with $\p{1-\frac{\tau_i}{\tau_{\max}}}c_i$, 
    where $\tau_{\max} = \max_{i \in \sA} \tau_i$.\;
\label{line:outlier-begin}

  For all $i$ with $c_i < \frac{1}{2}$, remove $i$ from $\sA$.\;
\label{line:outlier-end}

  Go back to line \ref{line:begin-loop}.\;
}
\protect\label{line:endif}
Let $W_1$ be the result of zeroing out all singular values of $W$ that are greater than $0.9$.\;

Let $Z = X_{\sA}W_0$, where $W_0 = (W-W_1)(I-W_1)^{-1}$.\;

\eIf{$\rank(Z) = 1$}{
  Output the average of the columns of $X_{\sA}$.
}{
  Output a column of $Z$ at random.
}
\end{algorithm}




==> finite-sample-old.tex <==
\subsection{Finite-Sample Concentration}

Our finite-sample concentration results will depend on three properties of the 
population distribution $p$:
\begin{itemize}
\item The \emph{$\epsilon$-quantile} $\tau_\epsilon$: this is the minimal threshold such that
      $\bP_{x \sim p}[\langle x - \mu, v \rangle \geq \tau_{\epsilon}] \leq \epsilon$ for all $\|v\| \leq 1$.
\item The \emph{conditional mean} $\rho_{\epsilon}$ of the $\epsilon$-quantile: 
      this is the minimal bound such that
      $\bE_{x \sim p}[\langle x - \mu, v \rangle \mid \langle v, x \rangle \geq \tau_{\epsilon}] \leq \rho_{\epsilon}$ for all $\|v\| \leq 1$. For distributions with light tails it will typically 
      be close to $\tau_{\epsilon}$, but in some cases can be much larger.
\item The \emph{$\epsilon$-quantile} $B_{\epsilon}$ of the norm: this is similar to $\tau_{\epsilon}$, but is now the minimal threshold such that $\bP_{x \sim p}[\|x - \mu\|_* \geq B_{\epsilon}] \leq \epsilon$.
\end{itemize}
Note that a distribution $p$ is $(\sigma,\epsilon)$-resilient if and only if 
$\sigma \leq \frac{\epsilon}{1-\epsilon}\tau_{\epsilon}$.

\begin{proposition}
Suppose that $p$ is $(\sigma.\epsilon)$-resilient, with norm quantiles $B_{\epsilon}$. 
Suppose that samples $x_1, \ldots, x_n$ are drawn independently from $p$. Then, for any 
$\epsilon_0 \leq \frac{1}{2}$, with probability $1-\delta$ 
%there is a set $S$ of $(1-\epsilon_0)n$ of the $x_i$ such that 
$S$ is $(\sigma', \epsilon)$-resilient with
\begin{equation}
\sigma' = \oo\p{\sigma + \int_{0}^{\epsilon_0} \tau_{t^2/\epsilon_0} dt},%\oo\p{\sigma + B_{\epsilon_0} \sqrt{\frac{\log(2/\delta)}{\epsilon^2 n}}}
\end{equation}
where $\epsilon_0 = \sqrt{\frac{\log(M/\delta)}{n}}$.
%for all $\epsilon \leq \epsilon_0$.
\end{proposition}
\begin{proof}
Take the assumed covering $v_1, \ldots, v_M$ of the unit ball. Fix 
some $\epsilon'$, and let $z_{ij} = \bI[\langle x_i - \mu, v_j] \geq \tau_{\epsilon'}$.
Note that $\bE[z_{ij}] = \epsilon'$ and $z_{ij} \in \{0,1\}$. By the Chernoff 
bound, for any fixed $j$, 
$\bP[\frac{1}{n} \sum_{i=1}^n z_{ij} \geq (1+t)\epsilon] \leq e^{-t\log(1+t)n\epsilon/2}$.
Setting the failure probability to $\delta/M$, we have 
\end{proof}


\subsection{[OLD] Finite-Sample Concentration}

In this section we establish Proposition~\ref{prop:concentration}.

\textbf{Preliminaries.} 
Recall that our goal is to bound 
\begin{equation}
\sup_{\|v\| \leq 1} \frac{1}{|S|} \sum_{i \in S} |\langle x_i - \mu, v \rangle|^k.
\end{equation}
Also recall the definition of $M$, as the size of the minimal set of vectors 
$v_1, \ldots, v_M$ such that $\max_{j=1}^M \langle v_j, x \rangle \geq \frac{1}{2} \sum_{\|v\| \leq 1} \langle v, x \rangle$ for all $x \in \bR^d$. Note that this implies that the 
convex hull of the $v_j$ contains the ball of radius $\frac{1}{2}$ under the norm 
$\|\cdot\|$, and hence 
\begin{equation}
\max_{j=1}^M \sum_{i \in S} |\langle x_i - \mu, v_j \rangle|^k \geq \frac{1}{2^k} \sup_{\|v\| \leq 1} \sum_{i \in S} |\langle x_i - \mu, v \rangle|^k.
\end{equation}
Using also the fact that $|S| \geq \frac{n}{2}$, we have
\begin{equation}
\label{eq:concentration-1}
\sup_{\|v\| \leq 1} \frac{1}{|S|} \sum_{i \in S} |\langle x_i - \mu, v \rangle|^k \leq 2^{k+1}\max_{j=1}^M \frac{1}{n} \sum_{i \in S} |\langle x_i - \mu, v_j \rangle|^k,
\end{equation}
and we will focus hereafter on bounding the max on the 
right-hand-side of \eqref{eq:concentration-1}.

\textbf{Potential function argument.}
We will consider the following potential function:
\begin{equation}
\psi(c) \eqdef \frac{1}{\lambda} \log\Big(\sum_{j=1}^M \exp\big(\frac{\lambda}{n} \sum_{i=1}^n c_i|\langle x_i - \mu, v_j \rangle|^k\big)\Big).
\end{equation}
Note that if $c \in \{0,1\}^n$ is the indicator function of a set $S$, then 
$\psi(c) \geq \max_{j=1}^M \frac{1}{n} \sum_{i \in S} |\langle x_i - \mu, v_j \rangle|^k$.

We initialize $c$ to $0$ and imagine going through the data in order from 
$x_1$ to $x_n$, at each point $i$ considering the effect of increasing $c_i$ from $0$ to $1$.
We will show that with reasonably high probability, increasing $c_i$ does not increase 
$\psi$ by too much, and hence there is a large enough set $S$ for which $\psi(c)$, and hence 
\eqref{eq:concentration-1}, is bounded.

Formally, the key inequality is the following. Let $w(c,j) = \exp\big(\frac{\lambda}{n} \sum_{i=1}^n c_i |\langle x_i - \mu, v_j \rangle|^k\big) / Z(c)$, where $Z(c)$ is chosen so that 
$\sum_{j=1}^M w(c,j) = 1$.
Also let $c_{+I}$ denote the vector obtained from $c$ by increasing $c_I$ by $1$. We then have
\begin{equation}
\label{eq:concentration-psi-ineq}
\psi(c_{+I}) - \psi(c) \leq \frac{1}{n} \sum_{j=1}^M w(c,j)|\langle x_I - \mu, v_j \rangle|^k + \frac{\lambda}{n^2} \sum_{j=1}^M w(c,j)|\langle x_I - \mu, v_j \rangle|^{2k}.
\end{equation}

In particular, suppose that $c^{(I-1)}$ is a vector chosen based only on $x_{1:I-1}$. Then
\begin{align}
\bE[\psi(c_{+I}^{(I-1)}) - \psi(c^{(I-1)}) \mid x_{1:I-1}] 
 &\leq \frac{1}{n} \sum_{j=1}^M w(c^{(I-1)},j) \bE[|\langle x_I - \mu, v_j \rangle|^k] + \frac{\lambda}{n^2} \sum_{j=1}^M w(c^{(I-1)},j) \bE[|\langle x_I - \mu, v_j \rangle|^{2k}] \\
 &\leq \frac{1}{n} \sum_{j=1}^M w(c^{(I-1)},j) \sigma_k^k + \frac{\lambda}{n^2} \sum_{j=1}^M w(c^{(I-1)},j) \sigma_{2k}^{2k} \\
 &= \frac{1}{n} \sigma_k^k + \frac{\lambda}{n^2} \sigma_{2k}^{2k}.
\end{align}
Now, we will update $c^{(I-1)}$ to $c^{(I)}$ based on $x_I$, as follows:
$c^{(I)} = c^{(I-1)}_{+I}$ if $\psi(c_{+I}^{(I-1)}) - \psi(c^{(I-1)}) \leq \frac{2}{\epsilon n}(\sigma_k^k + \frac{\lambda}{n} \sigma_{2k}^{2k})$, 
and otherwise $c^{(I)} = c^{(I-1)}$. This ensures that 
$\bE[\psi(c^{(I)}) - \psi(c^{(I-1)}) \mid x_{1:I-1}] \leq \frac{1}{n} (\sigma_k^k + \frac{\lambda}{n} \sigma_{2k}^{2k})$, and that it is at most 
$\frac{2}{\epsilon n} (\sigma_k^k + \frac{\lambda}{n} \sigma_{2k}^{2k})$ almost surely. 
Therefore, applying the Azuma-Hoeffding inequality, and using the 
fact that $\psi(0) = \frac{\log(M)}{\lambda}$, we have that
\begin{equation}
\bP\Big[\psi(c^{(n)}) \geq \frac{\log(M)}{\lambda} + (1+t)(\sigma_k^k + \frac{\lambda}{n} \sigma_{2k}^{2k}) \Big] \leq \exp(-\frac{t^2n\epsilon^2}{8}).
\end{equation}
Therefore, setting $t = 1$ and $\lambda = \sqrt{n/2\log(M)}$, we have 
\begin{equation}
\bP\Big[\psi(c^{(n)}) \geq 2\sigma_k^k + 2\sigma_{2k}^k \sqrt{\frac{2\log(M)}{n}}\Big] \leq \exp\big(-\frac{n\epsilon^2}{8}\big).
\end{equation}
Hence, with probability $\exp(-n/8\epsilon^2)$, $\psi$ is small enough. 
Moreover, each element $x_i$ is included in $S$ with probability at least 
$1-\epsilon/2$ by Markov's inequality. Therefore, the probability that 
$S$ has size at least $(1-\epsilon)n$ is also at most $\exp(-n\epsilon^2/8)$.
So, with probability at least $1 - 2\exp(-n\epsilon^2/8)$, we obtain a set 
$S$ of size at least $(1-\epsilon)n$ 
with the right-hand-side of \eqref{eq:concentration-1} bounded by 
$2^{k+2}(\sigma_k^k + \sigma_{2k}^k \sqrt{2\log(M)/n})$, which completes the 
proposition.

\textbf{Proof of \eqref{eq:concentration-psi-ineq}.} We finish by establishing the inequality 
\eqref{eq:concentration-psi-ineq}. The starting point is the following ``local norm bound'' 
for the log-sum-exp function, which is proved in Section 2.8 of \citet{shalev2011online}:
\begin{equation}
\label{eq:logsumexp-ineq}
\frac{1}{\lambda} \log(\sum_{j=1}^M \exp(\lambda s_j)) \leq \frac{1}{\lambda} \log(\sum_{j=1}^M \exp(\lambda t_j)) + \frac{\sum_{j=1}^M \exp(\lambda t_j)[(s_j - t_j) + \lambda (s_j - t_j)^2]}{\sum_{j=1}^M \exp(\lambda t_j)}.
\end{equation}
In our particular case, 
$t_j = \frac{1}{n} \sum_{i=1}^n c_i|\langle x_i - \mu, v_j \rangle|^k$, 
and $s_j - t_j = \frac{1}{n} |\langle x_I - \mu, v_j \rangle|^k$. Under this notation, 
we have $w(c,j) = \exp(\lambda t_j) / \sum_{j'=1}^M \exp(\lambda t_{j'})$, so that 
\eqref{eq:concentration-psi-ineq} exactly reduces to \eqref{eq:logsumexp-ineq}.



==> main-lp-proof.tex <==
\vskip -0.4in
\phantom{x}
\section{Proof of Theorem~\ref{thm:main-lp}}
\label{sec:main-lp-proof}

%\begin{proof}[Proof of Theorem~\ref{thm:main-lp}]
We first analyze the case when $\alpha \not\approx 1$. %Note that 
%For the first part, when $\alpha$ is small, first note that 
Lemma~\ref{lem:1st-moment-lp} and Proposition~\ref{prop:1st-2nd-lp} 
imply that if $|S| = \alpha n$ and $S$ is $(\sigma,\frac{1}{2})$-resilient 
in $\ell_p$-norm around $\mu$, then there is a set 
$S_0$ of size $\Omega(\alpha n)$ with second moments around $\mu$ bounded by 
$\oo\p{\sigma^2q}$ in $\ell_q$-norm. 
Letting $\mu'$ be the mean of $S_0$, Proposition~\ref{prop:recovery-lp} implies that with 
probability $\Omega(\alpha)$ we output a $\hat{\mu}$ with 
$\|\hat{\mu} - \mu'\|_p = \oo\p{\frac{\sigma}{\alpha} \sqrt{\frac{q}{p-1}}} = \oo\p{\frac{\sigma}{\alpha(p-1)}}$. 
Moreover, resilience of $S$ implies that $\|\mu - \mu'\|_p \leq \sigma$, hence 
$\|\hat{\mu} - \mu\|_p = \oo\p{\frac{\sigma}{\alpha(p-1)}}$ as well, as claimed.


For $\alpha \geq 0.87$, note that if $\sigmabest(\epsilon) \leq \sigma \sqrt{\epsilon}$ for 
$\epsilon \in [\frac{1-\alpha}{2}, \frac{1}{2}]$, 
then Proposition~\ref{prop:1st-2nd-lp-eps} and the following 
discussion imply that we can find a set $S_0$ of size $\alpha |S| = \alpha^2 n$ with 
$2$nd moments around $\mu$ bounded by $\oo\p{\sigma^2 q\log(\frac{1}{1-\alpha})}$. 
Therefore, Proposition~\ref{prop:recovery-lp} implies that we can output a $\hat{\mu}$ with 
$\|\hat{\mu} - \mu'\|_p = \oo\p{\sigma\sqrt{(1-\alpha^2)q\log(\frac{1}{1-\alpha})}} = \oot\p{\sigma \sqrt{q(1-\alpha)}}$, 
provided that $\alpha^2 \geq \frac{3}{4}$, which is true if $\alpha \geq 0.87$. 
In this case resilience of $S$ implies that 
$\|\mu - \mu'\|_p \leq \sigmabest(\frac{1-\alpha}{\alpha}) = \oo(\sigma\sqrt{1-\alpha})$,
so $\|\hat{\mu} - \mu\|_p = \oot\p{\sigma \sqrt{q(1-\alpha)}} = \oot\p{\sigma\sqrt{\frac{1-\alpha}{p-1}}}$ as well, which completes the proof. \hfill\BlackBox %\qed
%\end{proof}


==> notation.tex <==
\subsection*{Notation}

Given vectors $a_i$, we will let $A$ denote a matrix with $i$th column $a_i$, 
and let $A_T$ or $[a_i]_{i \in T}$ denote the submatrix with columns from $T$.
We let $X^{\dagger}$ be the pseudoinverse of $X$, and $\sigma_{k}(X)$ the $k$th 
singular value. % of $X$, and $X^{\dagger}$ the pseudoinverse. % of $X$.
Let $\bi$ denote the all-$1$s vector.
Given $p \in [1,2]$, we let $q \in [2,\infty]$ be such 
that $\frac{1}{p} + \frac{1}{q} = 1$.

For a $d \times n$ matrix $X$, we let $\|X\|_{p_1 \to p_2}$ denote $\max_{v \in \bR^n} \|Xv\|_{p_2} / \|v\|_{p_1}$. We let $\|X\|_2 = \|X\|_{2 \to 2}$ denote operator norm, 
and $\|X\|_F$ denote Frobenius norm.
Observe that $\|X\|_{2 \to p}^2 = \max_{\|v\|_q \leq 1} \sum_{i} |\langle x_i, v \rangle|^2$. 
%We will say that vectors $[x_i]_{i \in S}$ have $k$th moments bounded by $\sigma^k$ in 
%$\ell_q$-norm if 
%$\max_{\|v\|_q \leq 1} \frac{1}{|S|} \sum_{i \in S} |\langle x_i, v \rangle|^k \leq \sigma^k$. 


==> results.tex <==
\subsection*{Results}

%\todo{say somewhere around here that we're going to have multiple resilience notions, 
%one for each problem; we think this is a good way to think about robust estimation}

We consider the well-studied problem of robust mean estimation in the $\ell_2$-norm, 
then extend to the previously unstudied setting of estimation 
in $\ell_p$-norms (for $1 < p \leq 2$). We also give the first result on rank-$k$ estimation 
with error depending on $\sigma_{k+1}$ (the $k+1$st singular value)
%(the $k+1$st singular value of the data) rather than 
rather than $\sigma_2$. %\todo{save line?}

In each case, our argument takes the following form:
\begin{enumerate}
\setlength\itemsep{0em}
\item First, we formulate a basic resilience criterion such as 
      Definition~\ref{def:resilience-lp},      such that it 
      is clear that estimation/recovery is possible if we ignore computational constraints.
%\item If necessary, we ``power up'' the resilient set to a highly resilient core satisfying
%      additional properties.
\item Then, we develop an efficient algorithm based on the resilience criterion. 
      This typically involves minimizing a convex reconstruction error, then 
      removing outliers that cause the error to be too large.
\end{enumerate}
We found this separation of statistical and algorithmic concerns useful, and think 
it will likely prove fruitful for other robust learning problems as well (e.g. robust 
classification or regression). In our case, it seems to have led to substantially simpler 
algorithms and analyses relative to previous work.
%We show in Section~\ref{sec:info-theory} that Definition~\ref{def:resilience-lp} does 
%indeed straightforwardly  -- TODO include but move later

In addition, we found that resilient sets have a rich geometric structure, at least 
in the case of mean estimation. Up to constants, Definition~\ref{def:resilience-lp} is 
equivalent to having small first moments around $\mu$. Strikingly, we show that any 
resilient set also has a large core with bounded \emph{second} moments. 
This $L^1/L^2$ ``powering up'' result is crucial in enabling efficient estimation, 
because it allows us to work with convenient linear algebraic objects such as 
covariance matrices.

\paragraph{Results: mean estimation.} 
To start, we consider robust mean estimation in the $\ell_p$-norm. For our resilience criterion 
we use Definition~\ref{def:resilience-lp} above. % applied to the $\ell_p$-norm.
As we show in Section~\ref{sec:info-theory}, if we ignore computational efficiency then 
Definition~\ref{def:resilience-lp} directly enables robust mean estimation (the rough 
argument is that any two large resilient sets must have similar means).

Our main theorem on mean estimation in $\ell_p$ norms is the following:
Let $x_1, \ldots, x_n \in \bR^d$, and let $S \subseteq [n]$ be an unknown set 
whose mean we would like to estimate, with $|S| = \alpha n$. We have:
\begin{theorem}
\label{thm:main-lp}
Suppose that $S$ is $(\sigma,\frac{1}{2})$-resilient around $\mu$ in $\ell_p$-norm, 
with $p \in (1,2]$.
Then there is an efficient algorithm whose output $\hat{\mu}$
satisfies $\|\mu - \hat{\mu}\|_p = \oo\Big({\frac{\sigma}{\alpha(p-1)}}\Big)$ with 
probability $\Omega(\alpha)$.

Moreover, if $\alpha \geq 0.87$ and $S$ is $(\sigma\sqrt{\epsilon}, \epsilon)$-resilient 
for $\epsilon \in [\frac{1-\alpha}{2}, \frac{1}{2}]$, the same algorithm has
$\|\mu - \hat{\mu}\|_p = \oot\Big({\sigma\sqrt{\frac{1-\alpha}{p-1}}}\Big)$
with probability $1$.
\end{theorem}
The first part says that we can estimate the mean for any value of $\alpha$, 
even $\alpha < \frac{1}{2}$. The $\Omega(\alpha)$ success probability is necessary 
because the data could consist of $\frac{1}{\alpha}$ identical translates of $S$, in 
which case it is impossible to determine which one is correct.
The second part says that as $\alpha \to 1$, the estimation error goes to zero. 
%This is the first result to get meaningful guarantees in both of these regimes with 
%a single algorithm, even for $p = 2$.
Note that we can always replace the $\frac{1}{p-1}$ factor with $\log(d)$, since the 
$\ell_p$ and $\ell_{1 + \frac{1}{\log(d)}}$ norms are equivalent to within constant 
factors when $p$ is close to $1$.

En route to proving Theorem~\ref{thm:main-lp}, we establish the following 
geometric proposition, which allows us to replace the resilience 
criterion with a more convenient linear algebraic condition.
\begin{proposition}
\label{prop:powering-up-intro}
If $S$ is $(\sigma,\frac{1}{2})$-resilient in $\ell_p$-norm and $1 < p \leq 2$, 
then $S$ contains a set $S_0$ of size 
at least $\frac{1}{2}|S|$ with bounded 2nd moments:
$\|[x_i - \mu]_{i \in S_0}\|_{2 \to p} \leq 10\sigma\sqrt{\frac{|S_0|}{p-1}}$. 
\end{proposition}
We found this result quite striking --- while $(\sigma,\frac{1}{2})$-resilience is 
equivalent to having bounded 1st moments (see Lemma~\ref{lem:1st-moment-lp}), 
Proposition~\ref{prop:powering-up-intro} shows that we get a stronger 
2nd moment bound essentially for free. 
The fact that this can hold with no dimension-dependent factors is far from obvious.
In fact, if we replace 2nd moments with 3rd moments or take $p > 2$ then 
the analog of Proposition~\ref{prop:powering-up-intro} is false: we incur 
polynomial factors in the dimension even if $S$ is the standard basis of $\bR^d$
(see Section~\ref{sec:counterexample} for details).
The proof of Proposition~\ref{prop:powering-up-intro} involves 
minimax duality, Khintchine's inequality, and the strong convexity of $\ell_p$ norms.
We can also strengthen Proposition~\ref{prop:powering-up-intro} to yield $S_0$ 
of size $(1-\epsilon)|S|$.
%\todo{be more direct: we think this is a cool result, 
%get much stronger property than you thought;
%it's tempting to think this is obvious, but here's some things to give you pause}

\paragraph{Results: rank-$k$ recovery.}
Our final set of results relate to recovering a rank-$k$ approximation 
to the data in the presence of arbitrary outliers. We first define the goal:
given a set of points $[x_i]_{i \in S}$, let $X_S$ be the matrix whose 
columns are the $x_i$. 
Our goal is to obtain a low-rank matrix $P$ such that $\|(I-P)X_S\|_2$ is not much larger 
than $\sigma_{k+1}(X_S)$, where $\sigma_{k+1}$ denotes the $k+1$st singular value.

As before, we start by formulating an appropriate resilience criterion: 
\begin{definition}[Rank-resilience]
\label{def:resilience-rank-k}
A set of points $[x_i]_{i \in S}$ in $\bR^d$ 
is \emph{$\delta$-rank-resilient} if
%the matrix 
%$X = [x_i]_{i \in S}$ satisfies (i) $\sigma_{k+1}(X) \leq \sigma\sqrt{|S|}$
%and (ii) 
for all subsets $T$ of size at least 
$(1-\delta)|S|$, we have $\col(X_T) = \col(X_S)$ 
and $\|X_T^{\dagger}X_S\|_{2} \leq 2$, where $\dagger$ is the pseudoinverse and 
$\col$ denotes column space.
\end{definition}
Rank-resilience says that the variation in $X$ 
should be sufficiently spread out: there should not be a direction 
of variation that is concentrated in only a $\delta$ fraction of 
the points.

We can perform efficient rank-$k$ recovery even 
in the presence of a $\delta$ fraction of arbitrary data:
\begin{theorem}
\label{thm:main-rank-k}
Let $\delta\leq \frac{1}{3}$. 
If a set of $n$ points contains a set $S$ of size 
$(1-\delta)n$ that is $\delta$-rank-resilient, 
then there is an efficient algorithm
for recovering a matrix $P$ of rank at most $15k$
such that $\|(I-P)X_S\|_{2} = \oo(\sigma_{k+1}(X_S))$.
\end{theorem}
The power of Theorem~\ref{thm:main-rank-k} comes from the fact that 
the error depends on $\sigma_{k+1}$ rather than e.g.~$\sigma_2$, which 
is what previous results yielded.
This distinction is crucial in practice, since most data have a few 
(but more than one) large singular values followed by many small singular values. %that are much larger than the remainder.
Note that in contrast to Theorem~\ref{thm:main-lp}, Theorem~\ref{thm:main-rank-k} 
only holds when $S$ is relatively large: at least $(1-\delta)n$ in size.

